Mechanism Design for Crowdsourcing: An Optimal 1-1/e Competitive Budget-Feasible Mechanism for Large Markets

In this paper we consider a mechanism design problem in the context of large-scale crowdsourcing markets such as Amazon's Mechanical Turk, ClickWorker, CrowdFlower. In these markets, there is a requester who wants to hire workers to accomplish some tasks. Each worker is assumed to give some utility to the requester. Moreover each worker has a minimum cost that he wants to get paid for getting hired. This minimum cost is assumed to be private information of the workers. The question then is - if the requester has a limited budget, how to design a direct revelation mechanism that picks the right set of workers to hire in order to maximize the requester's utility. We note that although the previous work has studied this problem, a crucial difference in which we deviate from earlier work is the notion of large-scale markets that we introduce in our model. Without the large market assumption, it is known that no mechanism can achieve an approximation factor better than 0.414 and 0.5 for deterministic and randomized mechanisms respectively (while the best known deterministic and randomized mechanisms achieve an approximation ratio of 0.292 and 0.33 respectively). In this paper, we design a budget-feasible mechanism for large markets that achieves an approximation factor of 1-1/e (i.e. almost 0.63). Our mechanism can be seen as a generalization of an alternate way to look at the proportional share mechanism which is used in all the previous works so far on this problem. Interestingly, we also show that our mechanism is optimal by showing that no truthful mechanism can achieve a factor better than 1-1/e; thus, fully resolving this setting. Finally we consider the more general case of submodular utility functions and give new and improved mechanisms for the case when the markets are large.

==> intuition.tex <==
\section{Intuition} \label{sec.intuition}

We explain the high level idea of our mechanisms in this section for the additive utility functions. 
First we briefly explain the previous mechanisms designed for this problem, and then we introduce a new solution by developing on the previous ideas. 

\subsection{Uniform Allocation Rule} \label{sec.uniscalef}
A natural approach to this problem tries to find a single {\em cost per utility rate} (denoted by rate $r$) at which all the sellers get paid. Initially the buyer declares a very large rate $r$, and then sees which all sellers are willing to sell at this rate. If the total cost to buy from all these sellers at rate $r$ is higher than the budget $B$, then the buyer decreases the rate $r$. More formally, a natural descending price auction for this problem works as follows: 
\begin{enumerate}
\item Let $A$ denote the set of active sellers, and initially set $A=S$. \item Start with a very high rate $r$. 
\item Verify if all the active sellers can be paid with rate $r$, i.e. whether $r\cdot \sum_{i\in A} u_i \leq B$ or not. 
\item If the payment is feasible, then allocate the subset $A$, make the payment and stop. 
\item If the payment is not feasible, then decrease $r$ slightly, update $A$ accordingly by removing the sellers $i$ for whom $c_i/u_i > r$; Go to Step 3.
\end{enumerate}

Above auction is essentially the idea behind the {\em proportional share} mechanisms designed in \cite{2010-focs_singer_budget-feasible-mechanisms, 2011-soda_improved_budget_feasible}\footnote{
It is worth pointing out that for submodular utilities, they need to use an additional trick: constructing a (sorted) list of sellers in a greedy manner before running the auction.}, although they describe it in a forward auction format. One can easily see that the above auction is truthful, budget feasible, and in large markets achieve an approximation ratio of $\frac{1}{2}$ (with small modifications, this can be converted to a randomized $\frac{1}{2}$-approximation for arbitrary markets as well \cite{2011-soda_improved_budget_feasible}).

To develop this idea further, first think of the above mechanism by an associated allocation rule; we define this rule using a curve on the 2-dimensional plane, where the horizontal axis stands for the cost per utility rate, and the vertical axis stands for the allocation (so it will be from $0$ to $1$, and particularly $0$ or $1$ in case of integral assignments); Figure \ref{fig.uniform} depicts the curve for when the rate is $r$. 

\begin{figure}
\center
 \begin{tikzpicture}[scale=1] 
    %Draw axis
    \coordinate (y) at (0,3);
     \node at (0,3.2) {\tiny \textsf{Allocation}}; 
    \coordinate (x) at (5,0);
     \node at (5.2,-0.2) {\tiny \textsf{cost per utility rate}}; 
    \draw[axis] (y) -- (0,0) --  (x);
%    \draw [dashed] (0,1.1) -- (2.1,1.1) ;
%     \node at (-0.2,1.1) {$t$};
    \draw [ultra thick] (0,2) -- (4,2)  -- (4,0);
    \node at (-0.2,2) {$1$};
    \node at (4,-0.2) {$r$};    

%    \draw [dashed] (2.1,1.1) -- (2.1,0) ;
%    \node at (2.1,-0.2) {$t$};
 \end{tikzpicture}
 \caption{The Uniform Allocation Rule}
  \label{fig.uniform}
 \end{figure}
 
Locate each seller $i\in S$ on the point $c_i/u_i$ of the horizontal axis, and think of the allocation rule as the curve $f_r:\Real_+\to\{0,1\}$, so we have $f_r(x)=1$ if $x\leq r$ and $f_r(x)=0$ otherwise. For a fixed rate $r$, the allocation rule simply allocates all the sellers $i$ for whom $f_r(c_i/u_i)=1$. 

Call an allocation rule $f_r$ budget feasible if $r\cdot \sum_{i\in S} u_i\cdot f_r (c_i/u_i)\leq B$. Now, we can think of our previous mechanism in a simpler way: find the largest $r$ such that $f_r$ is budget feasible. As mentioned earlier, we can show that this mechanism has approximation ratio $\frac{1}{2}$ in large markets.\footnote{We can also provide a tight example: a large market in which the uniform allocation curve does not not achieve a ratio better than $\frac{1}{2}$} 
Rather than proving this claim here, we pose a more important question: Having defined $\{f_r\}_{r>0}$  as the family of uniform curves, we obtain a mechanism with approximation ratio $\frac{1}{2}$. 
Is it possible to design a more efficient mechanism using a different family of curves? If yes, which family leads to the best approximation ratio? We clarify this question further below.

\subsection{Non-Uniform Allocation Rules} \label{sec.nonuniscalef}
For any curve $f:\Real_+\to [0,1]$, we can define an associated family of curves 
\begin{align*}
\F(f)= \left\{f_r: \Real_+\to [0,1]\right\}_{r>0}
\end{align*}
 where $f_r$ denotes a curve which is same as $f$ except that it is stretched along the horizontal axis with ratio $r$, i.e. $f_r(x)=f(x/r)$ for all $x\geq 0$.

For any family $\F(f)$, we define an associated mechanism similar to the mechanism that we defined for the uniform curves: we pick the largest positive $r$ such that $f_r \in \F(f)$ is budget feasible. However, we yet need to define budget feasibility in the case of non-uniform curves. 
Similar to before, we say that the mechanism is budget feasible if the sum of its payments does not exceed $B$. However, we do not use identically the same payment rule as before, we use an extension of it which is inspired from the Myerson's payment rule\footnote{\label{myersonfnote}Myerson's Lemma \cite{myersonslemma} is a well-known lemma for designing truthful mechanisms; For any monotone allocation rule, it defines an associated payment rule that makes the mechanism truthful.}: Given an allocation rule $f_r$, the payments associated with it are defined to be
\begin{align*}
P_i(f_r) = u_i \cdot \left( b_i \cdot f_r(b_i) + \int_{b_i}^{\infty} f_r(x) \operatorname{d}x\right).
\end{align*}
where $b_i=c_i/u_i$.\footnote{In this section, we intentionally define $P_i$ as a function of $f_r$ (and not explicitly $c_i$); this is done since in here, we focus on $f_r$ as the more important factor for determining the payments. Obviously, the payments are still a function of $c_i$ as it can be seen in the definition.}
In words, the allocation rule allocates a fraction $f_r(b_i)$ of seller $i$ and the payment rule pays her $P_i(f_r)$. Fore more intuition, we have a visual description of the payment rule in Figure~\ref{fig.payment}; also, it is worth pointing out that when $f$ is uniform, then $P_i(f_r) = u_i \cdot r$, which coincides with our previous payment rule for uniform curves. 

 \begin{figure} 
\center
 \begin{tikzpicture}[scale=1] 
    %Draw axis
    \coordinate (y) at (0,3);
    \coordinate (x) at (5,0);
    \draw[axis] (y) -- (0,0) --  (x);
    
 \draw[black, ultra thick, domain=0:4] plot (\x, {1.2*ln(5-\x)});
\draw[dashed] (2.2,0) -- (2.2,{1.2*ln(5-2.2)});
\draw[ultra thick][dashed] (0,{1.2*ln(5-2.2)-0.01}) -- (2.2,{1.2*ln(5-2.2)-0.01});
\fill[fill=gray, opacity=0.2] (0,0) -- plot [domain=0:2.2] (\x,{1.2*ln(5-2.2)}) -- (2.2,0)  -- cycle;
\fill[fill=gray, opacity=0.2]  (2.2,0) -- plot [domain=2.2:4] (\x,{1.2*ln(5-\x)}) -- (4,0)  -- cycle;

    \node at (0,3.3) {$f_r$};
    \node at (-0.2,2) {$1$};
%    \node at (4,-0.2) {$1$};    
    \node at (2.3,-0.2) {${c_i}/{u_i}$};
 \end{tikzpicture}
 \caption{With allocation rule $f_r$, the payment to seller $i$ is defined to be $u_i$ times the shaded area under the curve.}
 \label{fig.payment}
 \end{figure}

Given the family of curves $\F(f)$, the mechanism associated with $\F(f)$, which we call \Scale$(f)$, is summarized below:
\begin{enumerate}
\item Find the largest positive number $r$ such that $f_r \in \F(f)$ is budget feasible.
\item For each seller $i\in S$, allocate a fraction $f_r(c_i/u_i)$ from seller $i$ and pay her $P_i (f_r)$.
\end{enumerate}


Unfortunately, \Scale($f$) is not truthful for all choices of $f$;\footnote{In fact, the uniform allocation rule is the only allocation rule that we could find for which \Scale($f$) is truthful.}
however, in Section \ref{sec.optmec}, we will be able to design a slightly different mechanism which is truthful for any continuous and decreasing choice of $f$.\footnote{The decreasing assumption on $f$ is required for truthfulness, roughly speaking, it is due to Myerson's Lemma.}
 In large markets, our truthful mechanism has {\em almost} the same allocation and payment rules as \Scale($f$), and so, it has almost the same approximation ratio as \Scale($f$) (assuming that the costs are truthfully reported to \Scale($f$)). 
 %In other words, in large markets, our truthful mechanism has the same approximation ratio 

%According to the above relation between \Scale($f$) and its corresponding truthful mechanism, we define a class of truthful mechanisms where each mechanism in this class is characterized by a decreasing and continuous allocation rule $f: \Real_+\to[0,1]$ and is the truthful mechanism corresponding to \Scale($f$). 
 
According to the above relation between \Scale($f$) and its corresponding truthful mechanism, we define a class of truthful mechanisms which contains, for any decreasing and continuous allocation rule $f: \Real_+\to[0,1]$, the truthful mechanism corresponding to \Scale($f$). Also, we pointed out that finding the optimal mechanism in this class is (roughly) equivalent to finding the optimal allocation rule for \Scale($f$). This motivates one of the main question that we ask in this paper: 
\begin{center}
Under what choice of $f$ does the mechanism \Scale($f$) reach its best performance?
\end{center}
%However, we will be able to design a slightly different mechanism which is truthful for any continuous and decreasing choice of $f$. Moreover, our truthful mechanism would still have the same approximation ratio as the original mechanism (when it is given the true costs). According to this fact, we insist on asking the question: what is the best choice of $(f)$?

So far, we know that when $f$ is the uniform allocation rule, the approximation ratio is $\frac{1}{2}$. To develop more intuition on this question, we devote the rest of this section to presenting a fairly simple choice of $f$, i.e. a step function, which leads to an improved approximation ratio. We fully answer this question in Sections \ref{sec.optimumf} and \ref{sec.hardness} by providing a choice of $f$ which achieves approximation ratio $1-1/e$ and proving that no other $f$ achieves a better ratio.  

\subsection{A First Improvement over the Uniform Allocation Rule}
The new allocation rule that we use is a step function denoted by $\mathsf{S}(t):\bbR_+\to[0,1]$ which is depicted in Figure \ref{fig.step}. We will prove that the mechanism which uses the family of curves $\mathcal{F} (\mathsf{S}(t))$ has approximation ratio $\approx 0.55$ for $t\approx 0.55$.
For expositional simplicity, we give a proof only for when all the sellers have unit utilities, i.e. $u_i=1$ for all $i\in S$; proof of the general case follows similarly. 

\begin{figure} 
\center
 \begin{tikzpicture}[scale=1] 
    %Draw axis
    \coordinate (y) at (0,3);
    \coordinate (x) at (5,0);
    \draw[axis] (y) -- (0,0) --  (x);
    \draw [dashed] (0,1.1) -- (2.1,1.1) ;
     \node at (-0.2,1.1) {$t$};
    \draw [ultra thick] (0,2) -- (2.1,2) -- (2.1,1.1) -- (4,1.1) -- (4,0);
    \node at (-0.2,2) {$1$};
    \draw [dashed] (2.1,1.1) -- (2.1,0) ;
    \node at (2.1,-0.2) {$t$};
    \node at (4,-0.2) {$1$};    
 \end{tikzpicture}
 \caption{The step allocation rule $\mathsf{S}(t)$}
 \label{fig.step}
 \end{figure}

We show that \Scale$(f)$ has approximation ratio $\approx 0.55$ when $f=\mathsf{Step}(t)$, for $t\approx 0.55$. However, for the analysis we keep $t$ as a parameter and will set its value at the end. For now, suppose that $f=\mathsf{Step}(t)$ for some positive $t<1$. 
We state a brief proof without going through details such as the tie-breaking rule.

Assume that $r=1$ is the largest $r$ for which $f_r$ is budget feasible; this assumption can be made w.l.o.g. by just normalizing the budget and costs. Then, suppose there are $m$ sellers $i\in S$ for whom $c_i/u_i \leq t$; we call these the {\em cheap} sellers. Also, suppose there are $n$ sellers $i\in S$ for whom $t < c_i/u_i \leq 1$, we call these the {\em expensive} sellers. 
These assumptions imply that the utility gained by our mechanism is $m+nt$. 
On the other hand, we prove that the optimum utility, $U^\star$, is at most $m(1+2t-t^2)+n$. After proving this, we optimize over $t$ to achieve the best approximation ratio. 

To give an upper bound on the optimum utility, first we write the budget in terms of $m,n,t$: see that $B=m (2t-t^2)+nt$, because \Scale($f$) pays $2t-t^2$ dollars per unit of utility to the cheap sellers (i.e. the area under the curve) and $1$ dollar per unit of utility to the expensive sellers. Given that the mechanism spends (almost) all of the budget, we get 
$B\approx m (2t-t^2)+nt$.

Now, we provide an upper bound on the maximum utility that can be earned with budget $B$. Suppose that the optimum solution earns all the cheap sellers for free, i.e. a total $m$ units of utility for free. 
Then, to earn the next $n$ units of utility, the optimum solution has to pay at least $nt$ dollars (for buying the $n$ expensive sellers). After that, the cost for any extra unit of utility is at least $1$, since for every other seller $i$, we have $c_i/u_i\geq 1$. Since the optimum solution has spent $nt$ dollars of the budget so far, then with the remaining $m (2t-t^2)$ dollars, it can earn at most $m (2t-t^2)$ units of utility. So, the total utility earned by the optimum solution is at most $m+n+m (2t-t^2)=m(1+2t-t^2)+n$. 

Consequently, the approximation ratio of \Scale($f$) is at at least $\frac{m+nt}{m(1+2t-t^2) + n}$. Now, see that 
\begin{align*}
\frac{m+nt}{m(1+2t-t^2) + n} \geq \min \left\{\frac{1}{1+2t-t^2}, t\right\}.
\end{align*}
To achieve the best ratio, we have to set $t$ such that $1/(1+2t-t^2)=t$; this gives $t\approx 0.55$  which improves the $0.5$-approximation ratio of the uniform curve. 




==> mechanism.tex <==

\section{A Class of Truthful Mechanisms} \label{sec.optmec}
In this section, we show how to convert \Scale($f$) to a {\em similar} mechanism which is individually rational, truthful, and budget feasible. 
\subsection{Preliminaries}
The {\em cost per utility rate} of a seller $i$ is defined by $c_i/u_i$; it is also simply called the {\em rate} of seller $i$ when there is no risk of confusion. 

\subsubsection*{Allocation Rules}
An allocation rule $f:\mathbb{R}^+\rightarrow [0,1]$ is a function using which we determine how much to buy from a seller. More precisely, the allocation rule $f$ is suggesting to buy $f(\frac{c_i}{u_i})$ units from seller $i$. For expositional simplicity, the domain of all the allocation rules in this paper is considered to be the {\em cost per utility rate}.\footnote{As opposed to defining the domain to be the cost, which is a typical way of defining allocation rules.} 
We do not enforce using the same allocation rule for all sellers.

We say an allocation rule $f$ is a {\em Standard Allocation Rule} if $f$ is a decreasing function such that $f:\Real^+\rightarrow [0,1]$, $f(0)=1$ and $f(e-1)=0$.\footnote{The choice of $e-1$ is just for simplifying the future calculations; it can be replaced with any other constant in the cost of a bit more complicated calculations} 

Given a standard allocation rule $f$ and a positive number $r$, the allocation rule $f_r$ is defined such that $f_r(rx)=f(x)$.
In simple words, $f_r$ is obtained by stretching $f$ along the horizontal axis with ratio $r$. When $f_r$ is clearly known from the context, we sometimes refer to $r$ by the {\em scaling ratio} for $f$. Finally, note that $f_r=f$ for $r=1$.



\subsubsection*{Payment Rules}
First, we define the notion of {\em \np{} rules}.
\Np{} rules are corresponding to allocation rules. The \np{} rule corresponding to the allocation rule $f_r$, is denoted by $Q_r:\bbR_+\to\bbR_+$ and is defined by:
\begin{align*}
Q_r (x)=x\cdot f_r(x) + \int_{x}^{\infty} f_r(y) \operatorname{d}y.
\end{align*}
Intuitively, $Q_r (x)$ just represents the area under the curve as we had seen before in Figure~\ref{fig.payment}.
The domain of $Q_r$ corresponds to the cost per utility rate (of sellers), and its range corresponds to payment per unit of utility.
More precisely, if a seller has cost per utility $x$,
then the payment to her is $Q_r(x)$ per unit of utility, e.g. if her item has utility $y$, they her total payment would be $y\cdot Q_r(x)$.


The payment to seller $i$ can be naturally defined from the \np{} rule.
Given the allocation rule $f_r$, its corresponding payment rule is denoted by $P_{i,r}:\bbR_+\to\bbR_+$ for seller $i$, and is defined by
\begin{align*}
P_{i,r}(x) = u_i \cdot Q_r(x/u_i),
\end{align*}
where $x$ denotes the cost reported by $i$.
This says, if allocation rule $f_r$ is used for seller $i$ and $f_r(c_i/u_i)$ units of her item is allocated, then the payment she receives is equal to $P_{i,r}(c_i)$.


\subsection{Description of the Mechanism}
Here, we first define Procedure \Scale($f$) formally, and then explain how to convert it to an individually rational, truthful, and budget feasible mechanism. In Section \ref{sec.optimumf}, by finding the best choice for $f$, we design such a mechanism with approximation ratio $1-1/e$.

Suppose we are given an allocation rule $f_r$ with corresponding payment rules $\{P_{i,r}\}_{i\in S}$. 
If for each seller $i$, we allocate a fraction $f_r(c_i/u_i)$ of her item and pay her $P_{i,r}(c_i)$, then it is straight-forward to verify that we get an individually rational and truthful mechanism (due to Myerson's Lemma). 
However, budget feasibility is not guaranteed, i.e. the sum of payments might exceed $B$. 
To overcome this issue, we {\em scale} the allocation rule with an appropriate ratio which guarantees budget feasibility. 

\begin{definition}
We say that allocation rule $f_r$ is a {\em \fit} rule if $\sum_{i\in S} P_{i,r} (c_i) = B$, i.e. the payments defined with respect to $f_r$ sum up to $B$.
\end{definition}

Given a standard allocation rule $f$, the mechanism starts with a very large scaling ratio $r=\infty$; so we would have $\sum_{i\in S} P_{i,r} (c_i) > B$. 

Then, the mechanism decreases $r$ until the rule $f_r$ becomes a \fit{} rule, namely, at point $r=\rstar$. The mechanism stops at this point and uses $f_{\rstar}$ and $\{P_{i,\rstar}\}_{i\in S}$ to determine the allocations and payments. The ratio $\rstar$ is also called the {\em stopping rate} of the mechanism. 
We address this process by Procedure \scale{} and define it below under the same name.

\begin{procedure}
\LinesNotNumbered
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{Standard Allocation Rule $f$, Budget $B$}
\Output{A scaling ratio $\rstar$}
\BlankLine

$r\leftarrow \infty$\;
%$f(x)\leftarrow \ln(e-x)$\;
\While {$f_r$ is not a \fit{} rule}{
	Decrease $r$ slightly\;
}
$\rstar\leftarrow r$\;
Output the scaling ratio $\rstar$\;
\caption{Scale($f$) {\label{alg.uniformratio}}}
\end{procedure}

In the while loop in Procedure \scale{}, we 
decrease the value of $r$ by a sufficiently small value.
We do not get into the details of formally defining these small decrements here. In fact, for many allocation rules $f$, (including our choice of $f$ which we will see later) the final stopping rate can be computed directly by solving an equation with a single unknown $\rstar$. We do not discuss the details in this section and simply assume that Procedure \ref{alg.uniformratio}($f$) has a polynomial running time.

Procedure \scale{} is clearly budget feasible, we can also prove that it is individually rational. But it indeed is not truthful; also, its efficiency depends on $f$. The two latter issues, however, are solvable: In the rest of this section, we show how to convert \scale{} to a truthful mechanism using a simple trick. After that, in Section \ref{sec.optimumf} we look into the more challenging question: What is the best choice for $f$?

We use a simple trick to convert Procedure \scale{} to a truthful mechanism. The idea is to define, for each seller $i$, an allocation rule which does not depend on $c_i$. In particular, we define the allocation rule for seller $i$ to be $f_{r_i}$, where $r_i$ will be chosen independently of $c_i$. 
For finding $r_i$, we run Procedure \scale{} on the instance which is obtained by setting $c_i$ to be $0$ while keeping cost of the other sellers intact; $r_i$ would be the stopping rate of the procedure. The formal definition of the truthful mechanism appears in Mechanism \ref{alg.truthful}.

\begin{algorithm}
\LinesNotNumbered
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{Standard Allocation Rule $f$, Budget $B$}
\BlankLine
%$f(x)\leftarrow \ln(e-x)$\;
\ForEach{$i\in S$}{
	$temp\leftarrow c_i$\;
	$c_i\leftarrow 0$\;
	$r_i\leftarrow $ \ref{alg.uniformratio}$(f)$\;
	$c_i\leftarrow temp$\;
}
\ForEach{$i\in S$}{
Allocate $f_{r_i}(c_i)$ from seller $i$\;
Pay $P_{i,r_i}(c_i)$ to seller $i$\;
}
\caption{The Truthful Mechanism {\label{alg.truthful}}}
\end{algorithm}

In Lemma \ref{lem.scalecanbegood}, we prove that Mechanism \ref{alg.truthful} is individually rational, truthful, and budget feasible. First, we state the following lemma which will be used in the proof.
%For simplicity in the analysis, w.l.o.g. we assume that sellers are sorted with respect to their cost per utility rate, i.e. $\frac{c_1}{u_1}\leq \ldots\leq \frac{c_n}{u_n}$. 
\begin{lemma} \label{lem.rdec}
For any seller $i\in S$ we have $\rstar\geq r_i$.
\end{lemma}
\begin{proof}
The proof is based on the fact that $P_{i,r}(x)$ is an increasing function of $r$ (for a fixed $x$) and 
is a decreasing function of $x$ (for a fixed $r$). 
The proof is by contradiction, suppose $\rstar < r_i$. 
Let $c'_j =c_j$ for all $j\in S\backslash\{i\}$ and let $c'_i=0$. Observe that 
\begin{align*}
B = \sum_{j\in S} P_{j,\rstar}(c_j) &\leq \sum_{j\in S} P_{j,\rstar}(c'_j)\\
&<  \sum_{j\in S} P_{j,r_i}(c'_j) 
\end{align*}
where the first inequality is due to the fact that $P_{j,\rstar}(x)$ is a decreasing function of $x$ and the second inequality is due to the fact that $\rstar < r_i$. However, note that the above inequalities imply that $B < \sum_{j\in S} P_{j,r_i}(c'_j)$, which contradicts with the budget feasibility of Procedure \scale{}: see that $\sum_{j\in S} P_{j,r_i}(c'_j)$ represents the payment of \scale{} when the costs are $c'_1,\ldots,c'_n$, and so it can not be larger than $B$.
\end{proof}

\begin{lemma} \label{lem.scalecanbegood}
Mechanism \ref{alg.truthful} is individually rational, truthful, and budget feasible.
\end{lemma}
\begin{proof}
Note that the allocation and payment rules for seller $i$, i.e. $f_{r_i}, P_{i,r_i}$, do not depend on the cost reported by her. 
This fact, along with the fact that $f_{r_i}$ is a monotone rule (decreasing function) implies individual rationality and truthfulness. The proof is almost identical to the proof of Myerson's Lemma and we do not repeat it here. 

The proof for budget feasibility needs a bit more work. 
Let $p_i, p'_i$ denote the payments to seller $i$ respectively in Mechanism \ref{alg.truthful} and Procedure \scale, i.e. $p_i = P_{i,r_i}(c_i)$ and $p'_i=P_{i,\rstar}(c_i)$.
The lemma is proved if we show that $p_i\leq p'_i$, since we have $\sum_{i\in S} p'_i = B$. 

To see $p_i\leq p'_i$, note that $P_{i,r}(x)$ is an increasing function of $r$ (for a fixed $x$). So, since we have $\rstar\geq r_i$ due to Lemma \ref{lem.rdec}, then $P_{i,r_i}(c_i) \leq P_{i,\rstar}(c_i)$. 
\end{proof}



\section{A ($1-1/e$)-Approximate Optimal Truthful Mechanism} \label{sec.optimumf}
So far, we have introduced a class of individually rational, truthful, and budget feasible mechanisms for the problem: Passing any standard allocation rule $f$ to Mechanism \ref{alg.truthful} makes an instance of the class which we denote by $\mathcal{M}_f$. 
Our goal in this section is finding the {\em most efficient} mechanism in this class. Formally, given a standard allocation rule $f$, we denote the approximation ratio of $\mathcal{M}_f$ by $\mathcal{R}_f$ and define it as:
\begin{align*}
\mathcal{R}_f=\inf_{{I}} \frac{\mathcal{U}_f ({I})}{\mathcal{U}^{\star}(I)},
\end{align*}
where the infimum is taken over all instances $I$ of the problem, 
$\mathcal{U}_f ({I})$ denotes the utility gained by $\mathcal{M}_f$ in instance $I$, and $\mathcal{U}^{\star}(I)$ denotes the optimum utility in instance~$I$.

The most efficient allocation rule $f$, is the one which maximizes $\mathcal{R}_f$. Our goal, in this section and Section \ref{sec.hardness}, is finding the most efficient allocation rule and its corresponding approximation ratio. Formally, we prove the following theorem.

\begin{theorem} \label{thm.main}
The most efficient (standard) allocation rule is $f(x)=\ln(e-x)$, for which we have $\mathcal{R}_f=1-1/e$, i.e. it has approximation ratio $1-1/e$.
\end{theorem}

We prove this theorem in two parts: In the first part we show that $\mathcal{R}_f\geq 1-1/e$ for $f(x)=\ln(e-x)$; this is proved in the current section. In the second part, we show that $\mathcal{R}_g\leq 1-1/e$ for any (standard) allocation rule $g$. This fact be seen as a consequence of our hardness result in Section \ref{sec.hardness}, 
which states that no truthful mechanism can achieve approximation ratio better than $1-1/e$. We also provide a more direct (alternative) proof in Section \ref{sec.lb} that shows our choice of $f(x)=\ln(e-x)$ is optimal among all possible choices of standard allocation rules.

%Now, we state a few definitions that are needed for the analysis. 

\subsection{Finding an optimal $f$ for the (non-truthful) Procedure \scale}
In this section, we prove that Procedure \scale{} has approximation ratio $1-1/e$ for $f(x)=\ln(e-x)$. 
Note that the Procedure \scale{} is not truthful, however its analysis will be helpful when analyzing our truthful mechanism in Section \ref{SEC.TRUTHU1} and in Section \ref{sec.generalu}.
Here, we analyze \scale{} assuming that the true costs are known; later, in Section \ref{SEC.TRUTHU1}, we use this result to prove that Mechanism \ref{alg.truthful} has approximation ratio $1-1/e$ for the same choice of $f$. 

\subsubsection{Preliminaries}
%First, we make a simplification of notation for the analysis in this section. Note that in Procedure \scale, the same allocation rule $f_{\rstar}$ is used for determining the allocation of all the sellers. So, the payment rule for two different sellers would be 

We use $g_r$ to denote the inverse of an allocation rule $f_r$, i.e. $g_r(x)=f_r^{-1}(x)$.
Given an allocation rule $f_r$, we also write an alternative definition of its corresponding \np{} rule $Q_r$. This definition, rather being in terms of $\frac{c_i}{u_i}$, would be in terms of $f_r(\frac{c_i}{u_i})$. This alternative definition is denoted by $G_r$, and is defined such that $Q_r(\frac{c_i}{u_i}) = G_r(f(\frac{c_i}{u_i}))$. In words, $G_r(x)$ represents the payment (per unit of utility) to a seller when a fraction $x$ of her item is allocated.
To be more precise, the payment per unit of utility to seller $i$ for allocating a fraction $y=f_r(\frac{c_i}{u_i})$ of her item is 
\begin{align*}
G_r(y)=\int_0^y g_r(x)\operatorname{d}x=Q_r(\frac{c_i}{u_i}).
\end{align*}
We also denote $g_1$ and $G_1$ respectively by $g$ and $G$.
%So, we would have $Q_r(\frac{c_i}{u_i}) = G_r(f(\frac{c_i}{u_i}))$.

\begin{proposition}
Given the standard allocation rule $f(x)=\ln(e-x)$, it is straight-forward to verify that $g(x)=e-e^x$ and $G(x)=ex-e^x+1$. Also, $f_r(x)=\ln\left(\frac{er-x}{r}\right)$.
\end{proposition}
From now on in this section, we assume that $f(x)=\ln(e-x)$.
Next, we prove a useful inequality in the following lemma which will be used in the analysis of \scale. 

\begin{lemma} \label{lem.key}
For any $x,\alpha$ such that $0\leq x,\alpha \leq 1$ we have
\begin{align*}
G(x)-\alpha\cdot g(x) \leq e\cdot (x-\alpha\cdot (1-{1}/{e})).
\end{align*}
\end{lemma}
\begin{proof}
%If $\alpha=0$, then we have
%\begin{align*}
%G(x)-\alpha\cdot g(x)= ex-e^x+1 \leq ex = e\cdot (x-\alpha\cdot (1-{1}/{e})).
%\end{align*}
%Also, if $\alpha=1$, then we have 
\begin{align*}
& \ \alpha (e^x-1) \leq e^x -1 \\
\Rightarrow &\ 
\alpha e^x -e^x +1 \leq \alpha\\
\Rightarrow &\ 
\alpha e^x -e^x +1 + e(x-\alpha)  \leq \alpha+ e(x-\alpha)\\
\textrm{\small (by the definition of $g, G$)\ }\Rightarrow &\ 
G(x)-\alpha\cdot g(x) \leq e\cdot (x-\alpha\cdot (1-{1}/{e})).
\end{align*}
\end{proof}

\subsubsection{Approximation Ratio of Procedure \scale}
In the following lemma, we prove the efficiency of Procedure \scale{} when all sellers report true costs.
\begin{lemma} \label{lem.key2approx}
If sellers report true costs, then Procedure \scale{} has approximation ratio $1-{1}/{e}$.
\end{lemma}
\begin{proof}
Observe that w.l.o.g. we can assume $\rstar=1$: If $\rstar\neq 1$, then we can construct a new instance which is {\em similar} to the original instance and has stopping rate $1$. More precisely, there exists some $\beta>0$ such that if we multiply the budget and the reported costs by $\beta$, the stopping rate becomes equal to $1$. Note that this operation will not change the optimal solution or the solution of \scale{} and can be performed w.l.o.g.

%the new instance would have the following 3 properties:
%\begin{enumerate}
%\item It has the same set of sellers with the same 
%\item \scale stops at rate $e$ in the new instance. 
%\item \scale allocates the same fraction from a seller in both instances, i.e. it still allocates a fraction $x_i$ from seller $i$ in the new instance. 
%\end{enumerate}
%This new instance can be constructed by simply scaling the budget $B$ and reported costs $c_i$ by an identical appropriate scaling  factor. 
Now, suppose that a fraction $x_i$ of item $i$ is allocated by \scale. 
Since $\rstar =1$, we can use Lemma \ref{lem.key} to write the following set of inequalities:
\begin{align*}
G(x_i)-\alpha_i \cdot g(x_i) \leq e\cdot (x_i-\alpha_i\cdot (1-{1}/{e})) &\hspace{1cm} \forall i\in S,
\end{align*}
where $\alpha_i$ is the fraction that is allocated from seller $i$ in the optimal solution (recall that we are are comparing \scale{} with the optimum fractional solution).
%iff $i\in S^*$ and $\alpha_i=0$ otherwise. 
The above inequalities can be multiplied by $u_i$ on both side and be written as:
\begin{align*}
u_i\cdot \left(G(x_i)-\alpha_i \cdot g(x_i)\right) \leq u_i\cdot e\cdot (x_i-\alpha_i\cdot (1-{1}/{e})) &\hspace{1cm} \forall i\in S.
\end{align*}
By adding up these inequalities, we get:
\begin{align}
\sum_{i\in S}u_i\cdot \left(G(x_i)-\alpha_i \cdot g(x_i)\right) \leq  e\cdot \sum_{i\in S} u_i\cdot \left(x_i-\alpha_i\cdot (1-{1}/{e})\right). \label{eq.addall}
\end{align}

Now, we show that if
\begin{align}
0\leq \sum_{i\in S}u_i\cdot \left(G(x_i)-\alpha_i \cdot g(x_i)\right),\label{eq.addallrhs}
\end{align}
then the lemma is proved using \eqref{eq.addall} and \eqref{eq.addallrhs}. First we show why \eqref{eq.addall} and \eqref{eq.addallrhs} prove the lemma, and then in the end, we prove \eqref{eq.addallrhs} itself.

Observe that \eqref{eq.addall}
and \eqref{eq.addallrhs} imply that 
\begin{align}
0 \leq  \sum_{i\in S} u_i\cdot\left(x_i-\alpha_i\cdot (1-{1}/{e})\right). \label{eq.2stepsb4}
\end{align}
Now, let  $U$ denote the utility gained by \scale{} and $\uopt = \sum_{i\in S}u_i \alpha_i$ denote the utility of the optimum (fractional) solution; see that \eqref{eq.2stepsb4} implies
\begin{align*}
(1-1/e)\cdot \uopt = \sum_{i\in S}\alpha_i u_i \cdot (1-{1}/{e}) \leq  \sum_{i\in S}x_i u_i = U,
\end{align*}
This would prove the lemma. 

So, it only remains to show that \eqref{eq.addallrhs} holds: First observe that $\sum_{i\in S}u_i\cdot G(x_i)=B$, since the sum represents the payment of \scale. Also, see that $\sum_{i\in S}\alpha_i u_i \cdot g(x_i) \leq B$, since this sum is a lower bound on the cost of the optimal solution, which is at most $B$. 
\end{proof}

\subsection{Special case: Analyzing our truthful mechanism for unit utilities}\label{SEC.TRUTHU1}
In this section, we prove that Mechanism \ref{alg.truthful} has approximation ratio $1-1/e$ in large markets when it uses the standard allocation rule $f(x)=ln(e-x)$ for the special case when all the utilities are equal to $1$. In other words, we will show that approximation ratio approaches $1-{1}/{e}$ as $\theta$, the market's largeness ratio, approaches $0$ for the case of unit utilities. The proof for the case of general utilities is intricate and appears in Section \ref{sec.generalu}.


Note that the assumption of unit utilities imply $c_i/u_i=c_i$ for any seller $i$. Next, we state two lemmas before proving the approximation ratio. For simplicity in the analysis, w.l.g., assume that $c_1 \leq c_2\leq \ldots \leq c_n$.

\begin{lemma}  \label{lem.rissorted}
$r_1 \geq r_2 \geq \ldots \geq r_n$. 
\end{lemma}
 
\begin{lemma} \label{lem.concave}
Let $u^\star(b):\bbR_+\to\bbR_+$ denote the maximum utility that the buyer can achieve with budget $b$ (when the items are divisible). Then, $u^\star(b)$ is concave function.
\end{lemma}

Proofs for both of these lemmas are straight-forward and are deferred to the appendix, Section \ref{sec.defferedproofs}.

\begin{comment}%%%%
\begin{lemma}
Mechanism \ref{alg.truthful} is budget feasible.
\end{lemma}
\begin{proof}
Let $p_i, p'_i$ denote the payments to seller $i$ respectively in Mechanism \ref{alg.truthful} and Procedure \scale. The lemma is proved if we show that $p_i\leq p'_i$, since we have $\sum_{i\in S} p'_i = B$. 

To see $p_i\leq p'_i$, note that $p_i=G_{r_i}(f_{r_i}(c_i))$ and $p'_i=G_{\rstar}(f_{\rstar}(c_i))$. Since $f(rx)$ and $G(rx)$ both are decreasing functions of $r$, and since $\rstar\geq r_i$ by Lemma \ref{lem.rdec}, then we have $G_{r_i}(f_{r_i}(c_i)) \leq G_{\rstar}(f_{\rstar}(c_i))$. 
\end{proof}
\end{comment}%%%%

\begin{lemma}
Mechanism \ref{alg.truthful} has approximation ratio $1-{1}/{e}$ when all the items have utility equal to $1$.
\end{lemma}
\begin{proof}
Recall that $\uopt=u^\star(B)$ and let $U$ denote the utility achieved by Mechanism~\ref{alg.truthful}. We need to show that $(1-1/e) \cdot \uopt \leq U$.
Instead of showing that $U=\sum_{i\in S} f_{r_i}(c_i)$ is large enough compared to $\uopt$, we show that $\sum_{i\in S} f_{r_n}(c_i)$ is large enough compared to $\uopt$; the lemma then would be proved since we have $f_{r_n}(c_i) \leq f_{r_i}(c_i)$ for all $i\in S$. To see why $f_{r_n}(c_i) \leq f_{r_i}(c_i)$, it is enough to note that $r_n\leq r_i$ due to Lemma \ref{lem.rissorted} which implies $f_{r_n}(c_i) \leq f_{r_i}(c_i)$.


We consider two cases for the proof: In Case~1 we assume $\cmax\leq \cbar$, and in Case~2 we assume otherwise, where the number $\cbar$ is the cost at which $f_{r_n}(\cbar)=1-1/e$, more precisely, this happens at $\cbar=r_n (e-e^{1-1/e})$. 

\paragraph{Case 1} In this case, observe that we have $f_{r_n}(c_i) \geq 1-1/e$ for all $i\in S$, which implies $f_{r_i}(c_i) \geq 1-1/e$. This just means $U \geq (1-1/e)n\geq (1-1/e)\uopt$.

\paragraph{Case 2} Let $U_n = \sum_{i\in S} f_{r_n}(c_i)$, we will show that 
\begin{align} 
U_n \geq (1-1/e)\cdot (1-o(1))\cdot \uopt. \label{eq.lun}
\end{align}
 To prove this, consider an auxiliary instance in which, instead of budget $B$, we have a reduced budget $B'=\sum _{i\in S} Q_{r_n}(c_i)$. Note that if we run Procedure \scale{} on the auxiliary instance, then its stopping rate is $r_n$, and so, the utility gained by the procedure is exactly $U_n$. 
Let $\uopt_{\aux}$ denote the optimal utility in the auxiliary instance. Then, by applying Lemma \ref{lem.key2approx} on the auxiliary instance, we have $U_n \geq (1-1/e)\cdot \uopt_{\aux}$.
So, if we show that 
\begin{align}
\uopt_{\aux}\geq (1-o(1))\cdot \uopt \label{eq.randomname}
\end{align}
then \eqref{eq.lun} holds and the proof is complete.

%For proving $\uopt_{\aux}\geq (1-o(1))\cdot \uopt$, we consider two cases: In Case~1, we assume $\cmax\leq \cbar$ and in Case~2 we assume otherwise, where the number $\cbar$ is the cost at which $f_{r_n}(\cbar)=1-1/e$, more precisely, this happens at $\cbar=r_n (e-e^{1-1/e})$. 
%\paragraph{Case 2} 
We use Lemma~\ref{lem.concave} to prove \eqref{eq.randomname}: First, we show that $B'\geq (1-o(1))\cdot B$; then, applying Lemma~\ref{lem.concave} would imply that  $u^\star(B')\geq (1-o(1)) \cdot u^\star(B)$, which is identical to \eqref{eq.randomname} by definition. So all we need to complete the proof is showing that $B'\geq (1-o(1))\cdot B$.

To this end, we prove that $B'\geq (1-\alpha \cdot \frac{\cmax}{B})\cdot B$, where $\alpha$ is a constant with value $(e-e^{1-1/e})^{-1}\approx 6/5$. This would prove the Lemma due to the large market assumption. First, observe that 
\begin{align}
B&=Q_{r_n}(0)+\sum_{i\in S\backslash\{n\}} Q_{r_n} (c_i) \leq Q_{r_n}(0)+B' \nonumber \\
&\Rightarrow B'\geq B-Q_{r_n}(0) \geq B-r_n.  \label{eq.bplb}
\end{align}
Now, recall that in Case 2, we have $\cmax\geq \cbar$, which implies
\begin{align}
B&\geq \cbar\cdot \frac{B}{\cmax} = r_n (e-e^{1-1/e})\cdot \frac{B}{\cmax} \nonumber\\
&\Rightarrow \cmax \cdot(e-e^{1-1/e})^{-1} \geq r_n. \label{eq.rnub}
\end{align}
Combining \eqref{eq.bplb} and \eqref{eq.rnub} implies $B'\geq (1-\alpha \cdot \frac{\cmax}{B})\cdot B$ with the promised value for $\alpha$.
\end{proof}
%\input{truthful.tex}


==> texmf.cnf.tex <==
TEXMFCNF = {$SELFAUTOLOC,$SELFAUTODIR,$SELFAUTOPARENT}{,{/share/texmf{-local,}/web2c}
